Probabilistic Models of Relational Implication

Relational data in its most basic form is a static collection of known facts. However, by learning to infer and deduct additional information and structure, we can massively increase the usefulness of the underlying data. One common form of inferential reasoning in knowledge bases is implication discovery. Here, by learning when one relation implies another, we can extend our knowledge representation. There are several existing models for relational implication, however we argue they are motivated but not principled. To this end, we define a formal probabilistic model of relational implication. By using estimators based on the empirical distribution of our dataset, we demonstrate that our model outperforms existing approaches. While previous work achieves a best score of 0.7812 AUC on an evaluatory dataset, our ProbE model improves this to 0.7915. Furthermore, we demonstrate that our model can be improved substantially through the use of link prediction models and dense latent representations of the underlying argument and relations. This variant, denoted ProbL, improves the state of the art on our evaluation dataset to 0.8143. In addition to developing a new framework and providing novel scores of relational implication, we provide two pragmatic resources to assist future research. First, we motivate and develop an improved crowd framework for constructing labelled datasets of relational implication. Using this, we reannotate and make public a dataset comprised of 17,848 instances of labelled relational implication. We demonstrate that precision (as evaluated by expert consensus with the crowd labels) on the resulting dataset improves from 53% to 95%.

==> ch_exp/subsec_models.tex <==
\subsection{Models of Relational Implication}

\subsubsection{Included Models}

We evaluate performance on a range of models:

\begin{description}
\item[Set based methods] DIRT, Cover and BInc.
\item[Cosine*] We use the cosine distance between embedded representations of relations.
\item[Entailment Graph]  
\item[ProbE] 
\item[ProbL*] Our full link-prediction model of probabilistic implication.
\end{description}



Here an asterisk indicates a model that requires a link prediction score. For all such techniques, we provide results using Model F\cite{riedel}, TransE \cite{transe}, DistMult \cite{distmult} and Complex \cite{complex}. For the $\cos$ score on the Complex model, we use the complex dot-product operation to calculate cosine similarity.

\subsection{Implication With Argument Permutation}
\label{subsec:permut}



==> ch_litreview/sec_ext.tex <==
\section{Other Work}

\subsubsection{Topic Modelling for Compatibility}


Context-sensitivity \cite{Melamud:2013tx}: use topic-modelling to make inference rules context-sensitive.
    
\subsubsection{Improving Embeddings through Known Implications}

\cite{Demeester:2016wa}



Demeester et al. 


==> dedication.tex <==
%%
%% Template dedication.tex
%%


\chapter{Dedication}

Peace in the world.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "thesis"
%%% End: 



==> listofpublications.tex <==
\chapter{List of Publications}

\begin{itemize}
\item[$\bullet$] insert author list \emph{insert paper title}.  (submitted to
	insert journal name)
\item[$\bullet$] insert author list \emph{insert paper title}.  
        insert journal name \textbf{insert volume number}, 
        insert article or page number (insert year)
\end{itemize}

